Alpha shapes in kernel density estimation

For every Gaussian kernel density estimator $f(x)=\sum_i a_i \exp(-\lVert x-x_i\rVert^2/2h^2)$ associated to a point cloud $\mathcal{D}=\{x_1,...,x_N\}\subset \mathbb{R}^d$, we define a nested family of closed subspaces $\mathcal{S}(a)\subset\mathbb{R}^d$, which we interpret as a continuous version of an alpha shape. Using arguments based on Fenchel duality, we prove that $\mathcal{S}(a)$ is homotopy equivalent to the superlevel set $\mathcal{L}(a)=f^{-1}[e^{-a},\infty)$, and that $\mathcal{L}(a)$ can be realized as the union of a certain power-shifted covering by balls with centers in $\mathcal{S}(a)$. By extracting finite alpha complexes with vertices in $\mathcal{S}(a)$, we obtain refined geometric models of noisy point clouds, as well as density-filtered persistent homology calculations. In order to compute alpha complexes in higher dimension, we used a recent algorithm due to the present authors based on the duality principle.

==> figures/colormaps.tex <==
\pgfplotsset{
colormap/species1/.style={%
    /pgfplots/colormap={species1}{%
      rgb=(0.0,.431,.114)
      rgb=(.302,.6745,.451)
      rgb=(.702,.863,.765)
      rgb=(1.0,1.0,.8)      
      rgb=(1.0,.8,.502)      
    },
  },
}

\pgfplotsset{
colormap/species2/.style={%
    /pgfplots/colormap={species2}{%
        rgb=(1.0,.8,.502) 
     rgb=(1.0,1.0,.8)  
      rgb=(.702,.863,.765)
          rgb=(.302,.6745,.451)
         rgb=(0.0,.431,.114)     
          rgb=(0.0,.431,.114)  
    },
  },
}

\pgfplotsset{
colormap/species3/.style={%
    /pgfplots/colormap={species3}{%
      rgb=(0.0,.431,.114)
      rgb=(.302,.6745,.451)
      rgb=(.702,.863,.765)
      rgb=(1.0,1.0,.8)      
      rgb=(1.0,.8,.502)      
            rgb=(1.0,.8,.502)      
    },
  },
}

\pgfplotsset{
colormap/species4/.style={%
    /pgfplots/colormap={species4}{%
        %rgb=(1.0,.8,.502) 
     rgb=(1.0,1.0,.8)  
      rgb=(.702,.863,.765)
          rgb=(.302,.6745,.451)
         rgb=(0.0,.431,.114)     
          rgb=(0.0,.431,.114)  
    },
  },
}

\pgfplotsset{
colormap/species4/.style={%
    /pgfplots/colormap={species4}{%
        rgb=(1.0,.8,.502) 
     rgb=(1.0,1.0,.8)  
      rgb=(.702,.863,.765)
          rgb=(.302,.6745,.451)
         rgb=(0.1,.431,.114)     
          rgb=(0,.3,.05)  
    },
  },
}

\pgfplotsset{
colormap/species5/.style={%
    /pgfplots/colormap={species5}{%
    rgb=(.451,.259,0.0)
        rgb=(.741,.549,.322) 
     rgb=(.969,.906,.776)  
      rgb=(.906,.871,.871)
          rgb=(.776,.906,.871)
         rgb=(.290,.710,.710)     
          rgb=(.094,.388,.290)  
    },
  },
}

\pgfplotsset{
colormap/species7/.style={%
    /pgfplots/colormap={species7}{%
        %rgb=(1.0,.8,.502) 
     rgb=(1.0,1.0,.8)  
     rgb=(1.0,1.0,.8) 
      %rgb=(.702,.863,.765)
       %rgb=(.702,.863,.765)
          %rgb=(.302,.6745,.451)
         %gb=(0.1,.431,.114)     
          %rgb=(0,.3,.05)  
    },
  },
}


\pgfplotsset{
colormap/species8/.style={%
    /pgfplots/colormap={species8}{%
        %rgb=(1.0,.8,.502) 
     %rgb=(1.0,.99,.925)  
     %rgb=(1.0,.99,.925) 
      rgb=(1.0,1.0,1.0)
       rgb=(1.0,1.0,1.0)
     %rgb=(.702,.863,.765)
     %rgb=(.702,.863,.765)
      %rgb=(.702,.863,.765)
       %rgb=(.702,.863,.765)
          %rgb=(.302,.6745,.451)
         %gb=(0.1,.431,.114)     
          %rgb=(0,.3,.05)  
    },
  },
}

\pgfplotsset{
colormap/plasma/.style={%
    /pgfplots/colormap={plasma}{%
      rgb=(0.050383, 0.029803, 0.527975)
      rgb=(0.186213, 0.018803, 0.587228)
      rgb=(0.287076, 0.010855, 0.627295)
      rgb=(0.381047, 0.001814, 0.653068)
      rgb=(0.471457, 0.005678, 0.659897)
      rgb=(0.557243, 0.047331, 0.643443)
      rgb=(0.636008, 0.112092, 0.605205)
      rgb=(0.706178, 0.178437, 0.553657)
      rgb=(0.768090, 0.244817, 0.498465)
      rgb=(0.823132, 0.311261, 0.444806)
      rgb=(0.872303, 0.378774, 0.393355)
      rgb=(0.915471, 0.448807, 0.342890)
      rgb=(0.951344, 0.522850, 0.292275)
      rgb=(0.977856, 0.602051, 0.241387)
      rgb=(0.992541, 0.687030, 0.192170)
      rgb=(0.992505, 0.777967, 0.152855)
      rgb=(0.974443, 0.874622, 0.144061)
      rgb=(0.940015, 0.975158, 0.131326)
    },
  },
}

\pgfplotsset{
colormap/species9/.style={%
    /pgfplots/colormap={species9}{%
        %rgb=(1.0,.8,.502) 
     %rgb=(1.0,.99,.925)  
     %rgb=(1.0,.99,.925) 
  %rgb=(.302,.6745,.451)
   %rgb=(.302,.6745,.451)
      %rgb=(.702,.863,.765)
       %rgb=(.702,.863,.765)
       rgb=(1.0,1.0,1.0)
       rgb=(1.0,1.0,1.0)
          %rgb=(.302,.6745,.451)
         %gb=(0.1,.431,.114)     
          %rgb=(0,.3,.05)  
    },
  },
}

\pgfplotsset{
colormap/species6/.style={%
    /pgfplots/colormap={species6}{%
    rgb=(.451,.259,0.0)
        rgb=(.741,.549,.322) 
     rgb=(.969,.906,.776)  
      rgb=(.906,.871,.871)
          rgb=(.776,.906,.871)
         rgb=(.290,.710,.710)     
          rgb=(.094,.388,.290)  
                    rgb=(.094,.388,.290) 
                    rgb=(.094,.388,.290) 
                       rgb=(.094,.388,.290) 
    },
  },
}

\pgfplotsset{
colormap/species6a/.style={%
    /pgfplots/colormap={species6a}{%
     rgb=(.094,.388,.290) 
       rgb=(.094,.388,.290) 
  rgb=(.094,.388,.290)
 rgb=(.094,.388,.290) 
 rgb=(.290,.710,.710)
rgb=(.776,.906,.871)
  rgb=(.906,.871,.871)
    rgb=(.969,.906,.776) 
         rgb=(.741,.549,.322) 
       rgb=(.451,.259,0.0)     
        },
  },
}

\pgfplotsset{
colormap/species6b/.style={%
    /pgfplots/colormap={species6b}{%
 rgb=(.094,.388,.290) 
 rgb=(.290,.710,.710)
rgb=(.776,.906,.871)
  rgb=(.906,.871,.871)
    rgb=(.969,.906,.776) 
         rgb=(.741,.549,.322) 
       rgb=(.451,.259,0.0)  
        rgb=(.451,.259,0.0)  
         rgb=(.451,.259,0.0)  
          rgb=(.451,.259,0.0) 
           rgb=(.451,.259,0.0)
        },
  },
}



\pgfplotsset{
colormap/pdpink0/.style={%
    /pgfplots/colormap={pdpink0}{%
        rgb=(1.0,.93,.9)  
        rgb=(1.0,.93,.9)     
    },
  },
}

\pgfplotsset{
colormap/pdblue0/.style={%
    /pgfplots/colormap={pdblue0}{%
        rgb=(.8,.9,1.0)  
        rgb=(.8,.9,1.0)     
    },
  },
}

\pgfplotsset{
colormap/pdpink1/.style={%
    /pgfplots/colormap={pdpink1}{%
        rgb=(1.0,.65,.6) 
        rgb=(1.0,.77,.73) 
        rgb=(1.0,.9,.87)  
        rgb=(1.0,.97,.95)  
    },
  },
}

\pgfplotsset{
colormap/pdblue1/.style={%
    /pgfplots/colormap={pdblue1}{%
        rgb=(.5,.75,1.0) 
        rgb=(.6,.8,1.0) 
        rgb=(.7,.85,1.0) 
        rgb=(.8,.9,1.0)  
    },
  },
}

\pgfplotsset{
colormap/bioheat/.style={/pgfplots/colormap={bioheat}{
rgb=(0.098039,0.290196,0.000000)
rgb=(0.415686,0.552941,0.082353)
rgb=(0.596078,0.713725,0.094118)
rgb=(0.882353,0.921569,0.364706)
rgb=(0.952941,0.674510,0.200000)
rgb=(0.937255,0.498039,0.156863)
rgb=(0.874510,0.227451,0.105882)
},
},
}


\pgfplotsset{
colormap/ising1/.style={/pgfplots/colormap={ising1}{
rgb=(0.396078,0.498039,0.839216)
rgb=(0.490196,0.545098,0.784314)
rgb=(0.580392,0.568627,0.682353)
rgb=(0.670588,0.596078,0.568627)
rgb=(0.756863,0.635294,0.423529)
rgb=(0.870588,0.654902,0.301961)
rgb=(0.917647,0.694118,0.239216)
},
},
}

\pgfplotsset{
colormap/ising2/.style={/pgfplots/colormap={ising2}{
rgb=(0.917647,0.694118,0.239216)
rgb=(0.870588,0.654902,0.301961)
rgb=(0.756863,0.635294,0.423529)
rgb=(0.670588,0.596078,0.568627)
rgb=(0.580392,0.568627,0.682353)
rgb=(0.490196,0.545098,0.784314)
rgb=(0.396078,0.498039,0.839216)
},
},
}


\pgfplotsset{
colormap/blackwhite/.style={/pgfplots/colormap={blackwhite}{
rgb=(.88,.88,.88)
rgb=(0.78,0.78,0.78)
rgb=(0.2,0.2,0.2)
rgb=(0.0,0.0,0.0)
},
},
}



       \pgfplotsset{
         colormap/seq1/.style={/pgfplots/colormap={seq1}{rgb=(0.839216,0.933333,0.960784)
         rgb=(0.615686,0.764706,0.823529)
rgb=(0.450980,0.654902,0.725490)
         rgb=(0.278431,0.529412,0.619608)
         rgb=(0.133333,0.431373,0.529412)
         },
         },
         }

\pgfplotsset{
         colormap/seq2/.style={/pgfplots/colormap={seq2}{
         rgb=(0.839216,0.933333,0.960784)
         rgb=(0.839216,0.933333,0.960784)
        rgb=(0.839216,0.933333,0.960784)
         rgb=(0.615686,0.764706,0.823529)
        rgb=(0.450980,0.654902,0.725490)
         rgb=(0.278431,0.529412,0.619608)
         rgb=(0.133333,0.431373,0.529412)
         },
         },
         }

\pgfplotsset{
colormap/bluered1/.style={/pgfplots/colormap={div1}{
rgb=(.1176,.188,.6235)
rgb=(.416,.549,.851)
rgb=(.729,.729,.733)
rgb=(.812,.447,.333)
rgb=(.573,.0,.039)
},
},
}


\pgfplotsset{
colormap/ising3/.style={/pgfplots/colormap={bluered1}{
rgb=(1.0,0,0)
rgb=(1,1,1)
rgb=(0,0,1)
},
},
}


\pgfplotsset{
colormap/div1/.style={/pgfplots/colormap={div1}{
rgb=(0.262745,0.545098,0.509804)
rgb=(0.654902,0.760784,0.643137)
rgb=(0.945098,0.925490,0.847059)
rgb=(0.905882,0.658824,0.466667)
rgb=(0.0.765,0.368627,0.203922)
},
},
}

\pgfplotsset{
colormap/div2/.style={/pgfplots/colormap={div2}{
rgb=(0.262745,0.545098,0.509804)
rgb=(0.654902,0.760784,0.643137)
rgb=(0.945098,0.925490,0.847059)
rgb=(0.905882,0.658824,0.466667)
rgb=(0.765,0.368627,0.203922)
rgb=(0.765,0.368627,0.203922)
rgb=(0.765,0.368627,0.203922)
rgb=(0.765,0.368627,0.203922)
},
},
}
